A Tale of Two Bases: Local-Nonlocal Regularization on Image Patches with Convolution Framelets

We propose an image representation scheme combining the local and nonlocal characterization of patches in an image. Our representation scheme can be shown to be equivalent to a tight frame constructed from convolving local bases (e.g. wavelet frames, discrete cosine transforms, etc.) with nonlocal bases (e.g. spectral basis induced by nonlinear dimension reduction on patches), and we call the resulting frame elements {\it convolution framelets}. Insight gained from analyzing the proposed representation leads to a novel interpretation of a recent high-performance patch-based image inpainting algorithm using Point Integral Method (PIM) and Low Dimension Manifold Model (LDMM) [Osher, Shi and Zhu, 2016]. In particular, we show that LDMM is a weighted $\ell_2$-regularization on the coefficients obtained by decomposing images into linear combinations of convolution framelets; based on this understanding, we extend the original LDMM to a reweighted version that yields further improved inpainting results. In addition, we establish the energy concentration property of convolution framelet coefficients for the setting where the local basis is constructed from a given nonlocal basis via a linear reconstruction framework; a generalization of this framework to unions of local embeddings can provide a natural setting for interpreting BM3D, one of the state-of-the-art image denoising algorithms.

==> notation.tex <==
\begin{table}[htbp]
\caption{Notations used throughout this paper}
\begin{center}% used the environment to augment the vertical space
% between the caption and the table
\begin{tabular}{c c p{10cm} }
\toprule
%\multicolumn{3}{c}{\underline{Symbols}}\\[.2em]
$I_k$ & & identity matrix in $R^{k\times k}$\\
$\vone_k$ & & vector with all one entries in $R^k$\\
%\multicolumn{3}{c}{}\\
%\multicolumn{3}{c}{\underline{General Notation}}\\[.2em]
$\left\| \cdot \right\|_{\mathrm{F}}$ & & matrix Frobenius norm\\
$\ell$ & & dimension of \emph{ambient space}, i.e. number of pixels in a patch\\
$p$ & & dimension of \emph{embedding space}, i.e. number of coordinate functions in the nonlocal embedding\\
$N$ & & number of data points (patches)\\
$X$ & & data matrix in $\mathbb{R}^{N\times \ell}$\\
$\t{X}$ & & embedded data matrix in $\mathbb{R}^{N\times p}$, ``orthogonalized" s.t. $\tX = \Phi_\embed\, C_\embed$\\
$X^i\, (\textrm{resp. }\t{X}^i)$ & & the $i$th coordinate in ambient space (resp. embedding space)\\
$\Phi_\embed$ & & normalized graph bases in $\mathbb{R}^{N\times p}$ from $\embed$ and $\Phi_\embed^{\top}\,\Phi_\embed = I_p$ \\
$\Phi$ & & full orthonormal nonlocal bases extended from $\Phi_\embed$\\
$C_\embed$ & & diagonal matrix with entries $\Vert \tX^i\Vert$\\
$x_i$ & & the $i$th row of $X$, i.e. the $i$th data point \\
$\tx_i$ & & embedding of $x_i$\\
$\embed$ &  & embedding function from $\mathbb{R}^{\ell}$ to $\mathbb{R}^p$\\
$\embed_x$ &  & affine approximation of $\embed$ at point $x$\\
%$\embed_x^{-1}$  & & pseudo inverse of $\embed_x$.\\
$V_0$ & & patch bases in $\mathbb{R}^{\ell\times p}$,\, s.t. $V_0^{\top}V_0 = I_p$.\\
$V$ & & full orthonormal local bases in $O(\ell)$\\
$C$ & & coefficient matrix\\
$f$ & & 1-D or 2-D signal, e.g. an image\\
$F$ & & patch matrix in $\mathbb{R}^{N\times \ell}$ generated from $f$, a special type of data matrix\\
$F_i$ & & $i$th patch\\
$F^i$ & & $i$th coordinate in patch space, e.g. $i$th pixel in all patches\\
$\t{F}$ & & embedded patch matrix \\
$\Psi $ & & bases in $\mathbb{R}^{N\times \ell}$ from $\phi_i\,v_j^{\top}$\\
$\psi $ & & bases in $\mathbb{R}^N$ from $\phi_i\,*v_j(-\cdot)$\\
$W$ & & affinity matrix of diffusion graph with Gaussian kernel\\
$D$ & & degree matrix from $W$\\
$L$ & & normalized graph diffusion Laplacian\\
$R_L$ & & graph operator in LDMM\\
\bottomrule
\end{tabular}
\end{center}
\label{tab: notation}
\end{table}

